Uniformity in $C^*$-algebras

We introduce a notion of a uniform structure on the set of all representations of a given separable, not necessarilly commutative $C^*$-algebra $\mathfrak{A}$ by introducing a suitable family of metrics on the set of representations of $\mathfrak{A}$ and investigate its properties. We define the noncommutative analogue of the notion of the modulus of continuity of an element in $C^*$-algebra and we establish its basic properties. We also deal with morphisms of $C^*$-algebras by defining two notions of uniform continuity and show their equivalence.

==> defin.tex <==

%%%%%%%%%% SPECIAL SYMBOLS AND MATHEMATICAL FONTS %%%%%%%%%%

\newcommand{\AAA}{\mathbb{A}}\newcommand{\BBB}{\mathbb{B}}\newcommand{\CC=
C}{\mathbb{C}}\newcommand{\DDD}{\mathbb{D}}
\newcommand{\EEE}{\mathbb{E}}\newcommand{\FFF}{\mathbb{F}}\newcommand{\GG=
G}{\mathbb{G}}\newcommand{\HHH}{\mathbb{H}}
\newcommand{\III}{\mathbb{I}}\newcommand{\JJJ}{\mathbb{J}}\newcommand{\KK=
K}{\mathbb{K}}\newcommand{\LLL}{\mathbb{L}}
\newcommand{\MMM}{\mathbb{M}}\newcommand{\NNN}{\mathbb{N}}\newcommand{\OO=
O}{\mathbb{O}}\newcommand{\PPP}{\mathbb{P}}
\newcommand{\QQQ}{\mathbb{Q}}\newcommand{\RRR}{\mathbb{R}}\newcommand{\SS=
S}{\mathbb{S}}\newcommand{\TTT}{\mathbb{T}}
\newcommand{\UUU}{\mathbb{U}}\newcommand{\VVV}{\mathbb{V}}\newcommand{\WW=
W}{\mathbb{W}}\newcommand{\XXX}{\mathbb{X}}
\newcommand{\YYY}{\mathbb{Y}}\newcommand{\ZZZ}{\mathbb{Z}}\newcommand{\kk=
k}{{\Bbbk}}%% the same as '\mathbb k'

\newcommand{\AAa}{\CMcal{A}}\newcommand{\BBb}{\CMcal{B}}\newcommand{\CCc}=
{\CMcal{C}}\newcommand{\DDd}{\CMcal{D}}
\newcommand{\EEe}{\CMcal{E}}\newcommand{\FFf}{\CMcal{F}}\newcommand{\GGg}=
{\CMcal{G}}\newcommand{\HHh}{\CMcal{H}}
\newcommand{\IIi}{\CMcal{I}}\newcommand{\JJj}{\CMcal{J}}\newcommand{\KKk}=
{\CMcal{K}}\newcommand{\LLl}{\CMcal{L}}
\newcommand{\MMm}{\CMcal{M}}\newcommand{\NNn}{\CMcal{N}}\newcommand{\OOo}=
{\CMcal{O}}\newcommand{\PPp}{\CMcal{P}}
\newcommand{\QQq}{\CMcal{Q}}\newcommand{\RRr}{\CMcal{R}}\newcommand{\SSs}=
{\CMcal{S}}\newcommand{\TTt}{\CMcal{T}}
\newcommand{\UUu}{\CMcal{U}}\newcommand{\VVv}{\CMcal{V}}\newcommand{\WWw}=
{\CMcal{W}}\newcommand{\XXx}{\CMcal{X}}
\newcommand{\YYy}{\CMcal{Y}}\newcommand{\ZZz}{\CMcal{Z}}

\newcommand{\AaA}{\EuScript{A}}\newcommand{\BbB}{\EuScript{B}}\newcommand=
{\CcC}{\EuScript{C}}
\newcommand{\DdD}{\EuScript{D}}\newcommand{\EeE}{\EuScript{E}}\newcommand=
{\FfF}{\EuScript{F}}
\newcommand{\GgG}{\EuScript{G}}\newcommand{\HhH}{\EuScript{H}}\newcommand=
{\IiI}{\EuScript{I}}
\newcommand{\JjJ}{\EuScript{J}}\newcommand{\KkK}{\EuScript{K}}\newcommand=
{\LlL}{\EuScript{L}}
\newcommand{\MmM}{\EuScript{M}}\newcommand{\NnN}{\EuScript{N}}\newcommand=
{\OoO}{\EuScript{O}}
\newcommand{\PpP}{\EuScript{P}}\newcommand{\QqQ}{\EuScript{Q}}\newcommand=
{\RrR}{\EuScript{R}}
\newcommand{\SsS}{\EuScript{S}}\newcommand{\TtT}{\EuScript{T}}\newcommand=
{\UuU}{\EuScript{U}}
\newcommand{\VvV}{\EuScript{V}}\newcommand{\WwW}{\EuScript{W}}\newcommand=
{\XxX}{\EuScript{X}}
\newcommand{\YyY}{\EuScript{Y}}\newcommand{\ZzZ}{\EuScript{Z}}

\newcommand{\Aa}{\mathfrak{A}}\newcommand{\Bb}{\mathfrak{B}}\newcommand{\=
Cc}{\mathfrak{C}}\newcommand{\Dd}{\mathfrak{D}}
\newcommand{\Ee}{\mathfrak{E}}\newcommand{\Ff}{\mathfrak{F}}\newcommand{\=
Gg}{\mathfrak{G}}\newcommand{\Hh}{\mathfrak{H}}
\newcommand{\Ii}{\mathfrak{I}}\newcommand{\Jj}{\mathfrak{J}}\newcommand{\=
Kk}{\mathfrak{K}}\newcommand{\Ll}{\mathfrak{L}}
\newcommand{\Mm}{\mathfrak{M}}\newcommand{\Nn}{\mathfrak{N}}\newcommand{\=
Oo}{\mathfrak{O}}\newcommand{\Pp}{\mathfrak{P}}
\newcommand{\Qq}{\mathfrak{Q}}\newcommand{\Rr}{\mathfrak{R}}\newcommand{\=
Ss}{\mathfrak{S}}\newcommand{\Tt}{\mathfrak{T}}
\newcommand{\Uu}{\mathfrak{U}}\newcommand{\Vv}{\mathfrak{V}}\newcommand{\=
Ww}{\mathfrak{W}}\newcommand{\Xx}{\mathfrak{X}}
\newcommand{\Yy}{\mathfrak{Y}}\newcommand{\Zz}{\mathfrak{Z}}

\newcommand{\aA}{\mathfrak{a}}\newcommand{\bB}{\mathfrak{b}}\newcommand{\=
cC}{\mathfrak{c}}\newcommand{\dD}{\mathfrak{d}}
\newcommand{\eE}{\mathfrak{e}}\newcommand{\fF}{\mathfrak{f}}\newcommand{\=
gG}{\mathfrak{g}}\newcommand{\hH}{\mathfrak{h}}
\newcommand{\iI}{\mathfrak{i}}\newcommand{\jJ}{\mathfrak{j}}\newcommand{\=
kK}{\mathfrak{k}}\newcommand{\lL}{\mathfrak{l}}
\newcommand{\mM}{\mathfrak{m}}\newcommand{\nN}{\mathfrak{n}}\newcommand{\=
oO}{\mathfrak{o}}\newcommand{\pP}{\mathfrak{p}}
\newcommand{\qQ}{\mathfrak{q}}\newcommand{\rR}{\mathfrak{r}}\newcommand{\=
sS}{\mathfrak{s}}\newcommand{\tT}{\mathfrak{t}}
\newcommand{\uU}{\mathfrak{u}}\newcommand{\vV}{\mathfrak{v}}\newcommand{\=
wW}{\mathfrak{w}}\newcommand{\xX}{\mathfrak{x}}
\newcommand{\yY}{\mathfrak{y}}\newcommand{\zZ}{\mathfrak{z}}

\newcommand{\aaA}{\mathscr{A}}\newcommand{\bbB}{\mathscr{B}}\newcommand{\=
ccC}{\mathscr{C}}\newcommand{\ddD}{\mathscr{D}}
\newcommand{\eeE}{\mathscr{E}}\newcommand{\ffF}{\mathscr{F}}\newcommand{\=
ggG}{\mathscr{G}}\newcommand{\hhH}{\mathscr{H}}
\newcommand{\iiI}{\mathscr{I}}\newcommand{\jjJ}{\mathscr{J}}\newcommand{\=
kkK}{\mathscr{K}}\newcommand{\llL}{\mathscr{L}}
\newcommand{\mmM}{\mathscr{M}}\newcommand{\nnN}{\mathscr{N}}\newcommand{\=
ooO}{\mathscr{O}}\newcommand{\ppP}{\mathscr{P}}
\newcommand{\qqQ}{\mathscr{Q}}\newcommand{\rrR}{\mathscr{R}}\newcommand{\=
ssS}{\mathscr{S}}\newcommand{\ttT}{\mathscr{T}}
\newcommand{\uuU}{\mathscr{U}}\newcommand{\vvV}{\mathscr{V}}\newcommand{\=
wwW}{\mathscr{W}}\newcommand{\xxX}{\mathscr{X}}
\newcommand{\yyY}{\mathscr{Y}}\newcommand{\zzZ}{\mathscr{Z}}

\newcommand{\aAA}{\pmb{A}}\newcommand{\bBB}{\pmb{B}}\newcommand{\cCC}{\pm=
b{C}}\newcommand{\dDD}{\pmb{D}}
\newcommand{\eEE}{\pmb{E}}\newcommand{\fFF}{\pmb{F}}\newcommand{\gGG}{\pm=
b{G}}\newcommand{\hHH}{\pmb{H}}
\newcommand{\iII}{\pmb{I}}\newcommand{\jJJ}{\pmb{J}}\newcommand{\kKK}{\pm=
b{K}}\newcommand{\lLL}{\pmb{L}}
\newcommand{\mMM}{\pmb{M}}\newcommand{\nNN}{\pmb{N}}\newcommand{\oOO}{\pm=
b{O}}\newcommand{\pPP}{\pmb{P}}
\newcommand{\qQQ}{\pmb{Q}}\newcommand{\rRR}{\pmb{R}}\newcommand{\sSS}{\pm=
b{S}}\newcommand{\tTT}{\pmb{T}}
\newcommand{\uUU}{\pmb{U}}\newcommand{\vVV}{\pmb{V}}\newcommand{\wWW}{\pm=
b{W}}\newcommand{\xXX}{\pmb{X}}
\newcommand{\yYY}{\pmb{Y}}\newcommand{\zZZ}{\pmb{Z}}

\newcommand{\aAa}{\pmb{a}}\newcommand{\bBb}{\pmb{b}}\newcommand{\cCc}{\pm=
b{c}}\newcommand{\dDd}{\pmb{d}}
\newcommand{\eEe}{\pmb{e}}\newcommand{\fFf}{\pmb{f}}\newcommand{\gGg}{\pm=
b{g}}\newcommand{\hHh}{\pmb{h}}
\newcommand{\iIi}{\pmb{i}}\newcommand{\jJj}{\pmb{j}}\newcommand{\kKk}{\pm=
b{k}}\newcommand{\lLl}{\pmb{l}}
\newcommand{\mMm}{\pmb{m}}\newcommand{\nNn}{\pmb{n}}\newcommand{\oOo}{\pm=
b{o}}\newcommand{\pPp}{\pmb{p}}
\newcommand{\qQq}{\pmb{q}}\newcommand{\rRr}{\pmb{r}}\newcommand{\sSs}{\pm=
b{s}}\newcommand{\tTt}{\pmb{t}}
\newcommand{\uUu}{\pmb{u}}\newcommand{\vVv}{\pmb{v}}\newcommand{\wWw}{\pm=
b{w}}\newcommand{\xXx}{\pmb{x}}
\newcommand{\yYy}{\pmb{y}}\newcommand{\zZz}{\pmb{z}}



%%%%%%%%%% MATHEMATICAL FUNCTIONS %%%%%%%%%%

\newcommand{\dens}{\operatorname{dens}}\newcommand{\diam}{\operatorname{d=
iam}}\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\ind}{\operatorname{ind}}\newcommand{\dist}{\operatorname{dis=
t}}\newcommand{\supp}{\operatorname{supp}}
\newcommand{\Inv}{\operatorname{Inv}}\newcommand{\Extr}{\operatorname{Ext=
r}}\newcommand{\conv}{\operatorname{conv}}
\newcommand{\dom}{\operatorname{dom}}\newcommand{\im}{\operatorname{im}}\=
newcommand{\id}{\operatorname{id}}
\newcommand{\cll}{\operatorname{cl}}\newcommand{\intt}{\operatorname{int}=
}\newcommand{\lin}{\operatorname{lin}}
\newcommand{\card}{\operatorname{card}}\newcommand{\Ann}{\operatorname{An=
n}}\newcommand{\Contr}{\operatorname{Contr}}
\newcommand{\Embed}{\operatorname{Embed}}\newcommand{\Iso}{\operatorname{=
Iso}}\newcommand{\Prob}{\operatorname{Prob}}
\newcommand{\Mes}{\operatorname{Mes}}\newcommand{\grad}{\operatorname{gra=
d}}\newcommand{\rbd}{\operatorname{rbd}}
\newcommand{\RAD}{\operatorname{RAD}}\newcommand{\sgn}{\operatorname{sgn}=
}\newcommand{\const}{\operatorname{const}}
\newcommand{\ord}{\operatorname{ord}}\newcommand{\Lip}{\operatorname{Lip}=
}\newcommand{\Metr}{\operatorname{Metr}}
\newcommand{\Auth}{\operatorname{Auth}}\newcommand{\Homeo}{\operatorname{=
Homeo}}\newcommand{\cov}{\operatorname{cov}}
\newcommand{\Emb}{\operatorname{Emb}}\newcommand{\SPAN}{\operatorname{spa=
n}}\newcommand{\comp}{\operatorname{comp}}
\newcommand{\mesh}{\operatorname{mesh}}\newcommand{\st}{\operatorname{st}=
}\newcommand{\Card}{\operatorname{Card}}
\newcommand{\Fix}{\operatorname{Fix}}\newcommand{\red}{\operatorname{red}=
}\newcommand{\tr}{\operatorname{tr}}
\newcommand{\rank}{\operatorname{rank}}\newcommand{\GCD}{\operatorname{GC=
D}}
\newcommand{\scalarr}{\langle\cdot,\mathrm{-}\rangle}
\newcommand{\scalar}[2]{\langle =
#1,#2\rangle}\newcommand{\leqsl}{\leqslant}\newcommand{\geqsl}{\geqslant}=

\newcommand{\continuum}{\cC}\newcommand{\RE}{\operatorname{Re}}\newcomman=
d{\IM}{\operatorname{Im}}
\newcommand{\epsi}{\varepsilon}\newcommand{\varempty}{\varnothing}\newcom=
mand{\dd}{\colon}
\newcommand{\dint}[1]{\,\textup{d} =
#1}\newcommand{\PARTIAL}[3][]{\frac{\partial_{#1} #2}{\partial #3}}
\newcommand{\quotient}[2]{\makebox[1ex][l]{\raisebox{1ex}{$#1$}}\makebox[=
1ex][l]{$\diagup$}\raisebox{-1ex}{$#2$}}
\newcommand{\inj}{\hookrightarrow}\newcommand{\surj}{\twoheadrightarrow}\=
newcommand{\bij}{\lhook\joinrel\twoheadrightarrow}



%%%%%%%%%% OFTEN USED PHRASES %%%%%%%%%%

\newcommand{\TFCAE}{The following conditions are equivalent:}
\newcommand{\tfcae}{the following conditions are =
equivalent:}\newcommand{\iaoi}{if and only if}
\hyphenation{U-ry-sohn Pa-ler-mo War-sza-wa Hil-bert-schen Hil-bert =
se-mi-groups spa-ces non-empty Ca-me-ron Le-bes-gue %%
   non-atomic}



%%%%%%%%%% REFERENCES TO \label AND BIBLIOGRAPHY %%%%%%%%%%

\newcommand{\REF}[1]{\textup{\ref{#1}}}\newcommand{\THM}[1]{Theorem~\text=
up{\ref{thm:#1}}}
\newcommand{\DEF}[1]{Definition~\textup{\ref{def:#1}}}\newcommand{\COR}[1=
]{Corollary~\textup{\ref{cor:#1}}}
\newcommand{\LEM}[1]{Lemma~\textup{\ref{lem:#1}}}\newcommand{\PRO}[1]{Pro=
position~\textup{\ref{pro:#1}}}
\newcommand{\REM}[1]{Remark~\textup{\ref{rem:#1}}}\newcommand{\EXM}[1]{Ex=
ample~\textup{\ref{exm:#1}}}
\newcommand{\EXS}[1]{Examples~\textup{\ref{exs:#1}}}\newcommand{\SUBL}[1]=
{Sublemma~\textup{\ref{sub:#1}}}
\newcommand{\PRB}[1]{Problem~\textup{\ref{prb:#1}}}



%%%%%%%%%% THEOREMS %%%%%%%%%%

\newenvironment{thm}[1]{\begin{Thm}\label{thm:#1}}{\end{Thm}}\newenvironm=
ent{lem}[1]{\begin{Lem}\label{lem:#1}}{\end{Lem}}
\newenvironment{cor}[1]{\begin{Cor}\label{cor:#1}}{\end{Cor}}\newenvironm=
ent{pro}[1]{\begin{Pro}\label{pro:#1}}{\end{Pro}}
\newenvironment{prp}[1]{\begin{Prp}\label{prp:#1}}{\end{Prp}}\newenvironm=
ent{dfn}[1]{\begin{Def}\label{def:#1}}{\end{Def}}
\newenvironment{exm}[1]{\begin{Exm}\label{exm:#1}}{\end{Exm}}\newenvironm=
ent{exs}[1]{\begin{Exs}\label{exs:#1}}{\end{Exs}}
\newenvironment{rem}[1]{\begin{Rem}\label{rem:#1}}{\end{Rem}}\newenvironm=
ent{rms}[1]{\begin{Rms}\label{rem:#1}}{\end{Rms}}
\newenvironment{com}[1]{\begin{Com}\label{com:#1}}{\end{Com}}\newenvironm=
ent{sub}[1]{\begin{Sub}\label{sub:#1}}{\end{Sub}}
\newenvironment{prb}[1]{\begin{Prb}\label{prb:#1}}{\end{Prb}}

